Training Dynamics of Softmax Self-Attention: Fast Global Convergence via Preconditioning

We study the training dynamics of gradient descent in a multilayer softmax self-attention network trained to perform linear regression and show that in the infinite-data limit this regression problem is equivalent to a matrix factorization problem. This connection motivates the design of Hera, a new first-order optimization algorithm for training self-attention networks. Key features of Hera include a reparameterization of the model arising from the matrix factorization geometry and a rescaling of the parameters which ensures that the empirical loss gradients remain close to the auxiliary matrix factorization gradients throughout training. Hera updates in the reparameterized model are equivalent to a certain preconditioned update in the original parameterization. We also propose a variant of Hera called Hera-PSD; our main theoretical result is that under small Gaussian initialization the excess risk of the model trained by Hera-PSD decreases exponentially fast in the number of gradient descent iterations, up to an additional error term that decreases as $1/n$, up to logarithmic factors, in the size of the training set. A particularly appealing aspect of our excess risk bound is that it does not degrade as the number of self-attention layers increases. In a stylized time-series prediction experiment in a nonlinear dynamical system, we find that a model trained by Hera achieves $98.1\%$ lower mean-squared test error than a model trained by AdamW and $97.7\%$ lower than a model trained by Muon at the same iteration budget.

==> body/reference_aliases.tex <==
% Compatibility keys for statements that have fixed-readout counterparts.
\makeatletter
\newcommand{\herareferencealias}[2]{%
  \AtEndDocument{%
    % Forward mathtools' citation marker so old eqref/noeqref keys still number
    % their replacement display on subsequent compilation passes.
    \@ifundefined{MT_r_#1}{}{%
      \protected@write\@auxout{}{\string\MT@newlabel{#2}}}%
    \@ifundefined{r@#2}{}{%
      \begingroup
      \expandafter\let\expandafter\hera@reference\csname r@#2\endcsname
      \protected@write\@auxout{}{\string\newlabel{#1}{\hera@reference}}%
      \endgroup}}}
% The depth-one statements are special cases of the all-depth theorem.
\herareferencealias{sec:single-layer}{sec:multi-layer}
\herareferencealias{thm:gd}{thm:multi-empirical}
\herareferencealias{eq:main-rate}{eq:multi-risk}
\herareferencealias{sec:single}{sec:multi}
\herareferencealias{sec:single-notation}{sec:multi-psd}
\herareferencealias{thm:gd-detailed}{thm:multi-empirical-detailed}
\herareferencealias{eq:algorithm}{eq:multi-update}
\herareferencealias{eq:initialization}{eq:multi-initialization}
\herareferencealias{eq:multi-chain-rule}{eq:hera-psd-gradients}
\herareferencealias{eq:multi-population-samples}{eq:multi-sample-conditions}
\herareferencealias{eq:param}{eq:v8-physical}
\herareferencealias{eq:physical-risk}{eq:fg-raw}
\herareferencealias{eq:popgradients}{eq:hera-psd-gradients}
\herareferencealias{eq:regularizer}{eq:fg-reg}
\herareferencealias{eq:single-prediction}{eq:v8-forward-normalized}
\herareferencealias{eq:single-risk-constant}{eq:multi-risk-constant}
\herareferencealias{eq:single-samples}{eq:multi-sample-conditions}
\herareferencealias{eq:single-tolerance}{eq:fg-grad}
\herareferencealias{eq:single-white}{eq:v8-normalization}
\herareferencealias{eq:v8-initial-data}{eq:data}
\herareferencealias{eq:v8-lifted-raw-gradients}{eq:hera-multilayer-gradient-residuals}
\herareferencealias{eq:v8-local-branch-derivative}{eq:multi-fixed-token}
\herareferencealias{eq:v8-physical-bound}{eq:fg-raw}
\herareferencealias{eq:v8-raw-gradients}{eq:hera-multilayer-gradient-residuals}
\herareferencealias{eq:v8-raw-mean-normalization}{eq:multi-unwhitened-convention}
\herareferencealias{eq:v8-single-errors}{eq:multi-normalized-error}
\herareferencealias{eq:v8-single-n0}{eq:multi-sample-conditions}
\herareferencealias{eq:v8-single-stats}{eq:fg-grad}
\herareferencealias{eq:v8-single-uniform}{eq:fg-grad}
\herareferencealias{rem:population-sensitivity}{sec:multi-risk-transfer}
\herareferencealias{sec:population-dependence}{sec:multi-risk-transfer}
\herareferencealias{sec:single-threshold}{sec:multi-convergence}
\herareferencealias{sec:v8-forward}{sec:multi-notation}
\herareferencealias{eq:multi-population-transfer}{eq:fg-raw}
\herareferencealias{eq:multi-regularizer}{eq:fg-reg}
\herareferencealias{eq:multi-uniform-gradient}{eq:fg-grad}
\herareferencealias{eq:multi-n0}{eq:multi-sample-conditions}
\herareferencealias{eq:multi-population-prefix}{eq:repar-multilayer-lifted-loss}
\herareferencealias{eq:multi-gamma}{eq:fg-score}
\makeatother

